Pauli Manipulation Detection codes and Applications to Quantum Communication over Adversarial Channels

We introduce and explicitly construct a quantum code we coin a "Pauli Manipulation Detection" code (or PMD), which detects every Pauli error with high probability. We apply them to construct the first near-optimal codes for two tasks in quantum communication over adversarial channels. Our main application is an approximate quantum code over qubits which can efficiently correct from a number of (worst-case) erasure errors approaching the quantum Singleton bound. Our construction is based on the composition of a PMD code with a stabilizer code which is list-decodable from erasures. Our second application is a quantum authentication code for "qubit-wise" channels, which does not require a secret key. Remarkably, this gives an example of a task in quantum communication which is provably impossible classically. Our construction is based on a combination of PMD codes, stabilizer codes, and classical non-malleable codes (Dziembowski et al., 2009), and achieves "minimal redundancy" (rate $1-o(1)$).

==> 1-intro.tex <==
\section{Introduction}

%A key challenge in quantum coding theory is that quantum noise is fundamentally continuous. Nevertheless, by focusing on discrete and highly structured error models, fairly general classes of quantum errors can be detected and corrected. In this work, we study a particularly natural form of quantum error detection for arbitrary Pauli errors, and we explore its application to tasks in quantum error correction and cryptography. To do so, we introduce and explicitly construct a class of quantum codes which detect arbitrary Pauli errors with high probability, regardless of their weight. 

%The very existence of quantum error-correcting codes was a major surprise, in part since quantum noise is fundamentally continuous. This challenge can also present an opportunity, to study quantum codes that can handle various restricted kinds of errors. In this paper, we consider quantum error-detection codes that can detect arbitrary Pauli errors (of arbitrarily large weight). This error model includes all bit-flip errors, and thereby captures all possible classical errors. 


The very existence of quantum error-correcting codes was a major surprise, in part since quantum noise is fundamentally continuous. This challenge can also present an opportunity, to study quantum codes that can handle various restricted kinds of errors. In this paper, we consider quantum error-detection codes that can detect arbitrary Pauli errors (of arbitrarily large weight). Their error model includes all bit-flip errors, and thereby captures all possible classical errors. 

%%Sam suggests
%In this paper, we consider quantum error-detection codes that can detect arbitrary Pauli errors with high probability. Note that unlike error-correcting codes, we do not need to limit the weight of the Paulis considered!

%Put this after mention AMD, and then you can say ``AMD codes require randomness in the encoding, whereas PMDs are deterministic...

We give an explicit construction of quantum codes which detect every Pauli error with high probability. By the previous remark, there is no direct (deterministic) classical analog of this result. Nevertheless, our codes resemble a well-known family of randomized classical codes known as algebraic manipulation detection codes (or AMDs) \cite{Cramer2008DetectionOA, Jafargholi2015TamperDA}. AMDs detect arbitrary additive errors (bit-flips), so long as the error is independent of the encoded message. Although this analogy can only go so far, inspired by their name, we refer to our codes as “Pauli Manipulation Detection” codes (or PMDs):\footnote{See \Cref{def:PMD2} for a formal definition. $\|\cdot\|_\infty$ is the operator norm, or Schatten infinity norm. }

%In this work, we introduce and explicitly construct a new class of quantum codes which detect every Pauli error with high probability. By the previous remark, there is no direct (deterministic) classical analog of this result. Nevertheless, our codes resemble a well-known class of classical “tamper-detection” codes known as algebraic manipulation detection codes (or AMDs) \cite{Cramer2008DetectionOA, Jafargholi2015TamperDA}. AMDs detect arbitrary additive errors (bit-flips), so long as the error does not depend on the encoded message. Although this analogy can only go so far, inspired by their name, we refer to our codes as “Pauli Manipulation Detection” codes (or PMDs):\footnote{See \Cref{def:PMD2} for a formal definition. $\|\cdot\|_\infty$ is the operator norm, or Schatten infinity norm. }


\begin{definition} 
We refer to a subspace $\Pi$ of an $n$-qubit Hilbert space as an $\epsilon$-$\PMD$ if, for every $n$-qubit Pauli error $E\neq \mathbb{I}$, 
\begin{equation}
    \|\Pi E\Pi\|_\infty\leq \epsilon.
\end{equation}
\end{definition}

This definition implies that every Pauli error on the code is detected \textit{almost}-\textit{deterministically}: if a code-state $\ket{\psi}\in \Pi$ is corrupted by a Pauli error $E\neq \mathbb{I}$, the projective measurement onto the PMD code-space $(\Pi, \mathbb{I}-\Pi)$ does not detect the Pauli tampering with probability at most
\begin{equation}
 \bra{\psi}E^\dagger \Pi E \ket{\psi} \leq \|\Pi E^\dagger \Pi E\Pi \|_\infty = \|\Pi E\Pi\|^2_\infty\leq \epsilon^2.
\end{equation}
% By the GML...
The gentle-measurement lemma then implies that PMD codes are able to detect whether they were corrupted by a Pauli, without disturbing the corrupted code-state. That is, conditioned on measuring $\mathbb{I}-\Pi$,
\begin{equation}
    (\mathbb{I}-\Pi) E \ket{\psi} \approx E\ket{\psi}. 
\end{equation}
%%% Sam
We leverage this key idea to construct the first efficient quantum codes approaching the information-theoretically optimal rate (or ``minimal redundancy") for two tasks in quantum coding theory and cryptography.

Our main application is an approximate quantum code over qubits for the adversarial erasures channel, which is able to efficiently correct from a near-optimal number of erasure errors. Due to a well-known connection between quantum error correction and secret sharing \cite{Gottesman1999TheoryOQ, Cleve1999HOWTS, Smith2000QuantumSS, Crpeau2005ApproximateQE}, this result can be understood as a quantum secret sharing scheme with qubit shares. Our second application is a quantum authentication code over ``qubit-wise" channels, which does not require a secret key. Curiously, these codes provide a form of keyless authentication which is provably impossible with classical messages.



%\begin{itemize}
%    \item An approximate quantum code over qubits for the adversarial erasures channel, which is able to efficiently correct from a near-optimal number of erasure errors.\footnote{Equivalently, this result can be understood as quantum secret sharing scheme with \emph{qubit shares} \cite{Gottesman1999TheoryOQ, Cleve1999HOWTS, Smith2000QuantumSS, Crpeau2005ApproximateQE}.}
%    \item A quantum authentication code over ``qubit-wise" channels, which does not require a secret key. Curiously, these codes provide a form of keyless authentication which is provably impossible with classical messages.
%\end{itemize}
%SAM: Explain what ``qubit-wise'' means here or in bullet!

%%%
%We find that this simple idea, that PMD codes detect Pauli errors while approximately preserving the corrupted code-state, really captures the power behind our definition. In this work, we show how to use PMD codes, combined with stabilizer quantum error correction \cite{Gottesman1997StabilizerCA}, to construct the first efficient quantum codes which approach the information-theoretically optimal rate (or ``minimal redundancy") for two tasks in quantum coding theory and cryptography:

%We emphasize that although these codes only offer error-detection or ``authentication" for Pauli channels, in contrast to generic quantum authentication codes \cite{barnum2002authentication}, they do so without assuming a random secret key shared between sender and receiver. In fact, they do not require any randomness at all.\footnote{While the absence of shared randomness is a feature of both classical and quantum tamper-detection codes, the absence of any randomness (i.e. pure state encodings) has only been observed in select few quantum tamper-detection codes \cite{Boddu2021TamperDA}.} In this work, we show how to use $\PMD$ codes, combined with stabilizer quantum error correction \cite{Gottesman1997StabilizerCA}, to remove the need for shared randomness in two settings where randomness was previously believed to be necessary. In doing so, we are able to achieve the information-theoretically optimal rate, or ``minimal redundancy", for the coding tasks we study.

%Our main application is an approximate quantum code over qubits for the adversarial erasures channel, which is able to efficiently correct from a near-optimal number of erasure errors. Due to a well-known connection between quantum error correction and secret sharing \cite{Gottesman1999TheoryOQ, Cleve1999HOWTS, Smith2000QuantumSS, Crpeau2005ApproximateQE}, this result can be understood as quantum secret sharing scheme with minimal-sized (qubit) shares. Our second application is a quantum authentication code over ``qubit-wise" channels, which does not require a secret key. Curiously, these codes provide a form of keyless authentication which is provably impossible with classical messages.



\subsection{Our Results}

\subsubsection{Constructions of PMD codes} 

Our first result is an explicit construction of PMD codes, which achieves rate near $1$ and inverse-exponential error. 

\begin{theorem}\label{theorem:results-pmdexplicit}
    For all sufficiently large integers $n$ and $\lambda | n$, there exists an $\epsilon$-$\PMD$ encoding $n-\lambda$ qubits into $n$ qubits with error $\epsilon \leq n^{1/2}\cdot 2^{1-\lambda/4}$. Moreover, it can be constructed and encoded efficiently.
\end{theorem}

Our construction is based on the stabilizer ``Purity Testing" codes (PTCs) introduced by \cite{barnum2002authentication} in the context of quantum message authentication. Informally, a PTC is a pseudorandom set of stabilizer codes $\{Q_k\}_{k\in K}$ \cite{Gottesman1997StabilizerCA} which detects every Pauli error with high probability (over random choice of the key $k$). We show that the natural approach of encoding\footnote{$\Enc_\PMD$ and the $\Enc_{Q_k}$ are unitaries, acting on a message register and ancilla qubits initialized to $\ket{0}$ (omitted for clarity).} a message state $\ket{\psi}$ into a superposition of PTC encodings,
\begin{equation}
    \Enc_\PMD\ket{\psi} = |K|^{-1/2}\sum_{k\in K}\ket{k}\otimes \Enc_{Q_k}\ket{\psi},
\end{equation}
\textit{almost} defines a PMD. Unfortunately, in general this construction is not a PMD. However, we show that the family of PTC's designed in \cite{barnum2002authentication} satisfy a certain form of ``key manipulation security", which guarantees this construction is secure (and maybe of independent interest). 

We complement our explicit code constructions with randomized (Monte Carlo) constructions of $\PMD$ codes from $t$-designs. A $t$-design is a distribution over unitaries which ``resembles" the first few moments of the Haar measure, and can be thought of a derandomization of a uniformly random unitary. 

\begin{theorem}
    Hi
\end{theorem}

By appealing to known constructions of (approximate) $t$-designs from random quantum circuits, we arrive at the intriguing conclusion that that geometrically-local, linear-depth random quantum circuits are $\PMD$ codes. 

Our first application of PMD codes is to approximate quantum error correction.

\subsubsection{Approximate Quantum Erasure Codes on the Quantum Singleton Bound}
\label{section:aqec-result}

An erasure error (or detectable leakage) on a quantum error correcting code corresponds to an error on a known location of the code. Erasure correction has recently found renewed interest in the quantum computing community, due to connections with quantum secret sharing \cite{Cleve1999HOWTS}, fault tolerance \cite{Wu2022ErasureCF}, the information-disturbance tradeoff \cite{Kretschmann2006TheIT}, and even information retrieval in black holes \cite{Yoshida2017EfficientDF}.

The quantum Singleton or ``no-cloning" bound imposes an information-theoretic limit on the maximum number of erasures a quantum code can (even approximately) correct from. It states that no quantum code of rate $r$ can correct from more than a $\frac{1}{2}(1-r)+o(1)$ fraction of erasures, for any assymptotically small approximation error \cite{Knill1996TheoryOQ, Rains1997NonbinaryQC, Grassl2020EntropicPO}. Moreover, to approach this bound over small alphabet sizes, one fundamentally needs \textit{approximate} quantum error correction: A famous result by Rains \cite{Rains1996QuantumSE} showed that no exact quantum code on qubits can correct from more than even a $1/3$ fraction of erasures. 

Our main result in this work is a randomized construction of efficient and near-optimal approximate quantum
code over qubits for the adversarial (worst-case) erasures channel.

\begin{theorem}[Main Result]\label{theorem:main}
    For every rate $0<r<1$ and sufficiently large $n\in \mathbb{N}$, there exists a Monte Carlo construction of an $n$ qubit quantum code of rate $r$ which corrects from a fraction $\delta\geq \frac{1}{2}(1-r) - O(\log^{-1} n)$ of erasures, up to an inverse-exponentially small recovery error $\epsilon = 2^{-\Tilde{\Omega}(n)}$. The construction succeeds with probability $1-2^{-\Tilde{\Omega}(n)}$.
\end{theorem}

Moreover, one can encode, decode, and sample a classical description of our codes efficiently in poly$(n)$ time. 

A challenging consequence of the relaxation to approximate erasure correction is that non-adaptive (or oblivious) adversaries are fundamentally very different than adaptive adversaries \cite{Lin2018SecretSW}, which can use the erased qubits to learn partial information about the message (and modify their corruption). While against the former one can often borrow ideas from the well-studied random erasure error model \cite{Hayden2017ApproximateQE, Gullans2020QuantumCW}, in the adaptive setting we require very different techniques.

Our code construction is based on a recent approach to design quantum codes against adversarial errors, list-decodable stabilizer codes \cite{Leung2006CommunicatingOA, Bergamaschi2022ApproachingTQ}. However, known approaches to use list decoding for approximate quantum error correction either assume shared randomness between sender and receiver, or require a large qu\textit{d}it alphabet size. Thereby, they are unable to approach the quantum Singleton bound over qubits, at least in a ``one-shot" setting.
% Sam: remove last sentence

Our new insights lie in combining our PMD codes, with a new type of stabilizer code which is list-decodable \textit{from erasures}, an analog to the classical notion introduced by \cite{Guruswami2001ListDF}. In this application, our main technical contribution is a reduction from approximate quantum erasure correction to PMDs and erasure list-decoding, and is inspired by a classical result by \cite{Cramer2015LinearSS} on the construction of classical secret sharing schemes from AMDs and list-decodable codes.  

%Our code construction is based on a promising recent approach to design approximate quantum codes, list-decodable stabilizer codes \cite{Leung2006CommunicatingOA, Bergamaschi2022ApproachingTQ}. However, known approaches to use list decoding for approximate quantum error correction either assume shared randomness between sender and receiver, or require a large qu\textit{d}it alphabet size. Thereby, fundamentally, they are unable to construct erasure codes over qubits. 

%Our key new insight lies in wrapping our PMD codes with a stabilizer code which is list-decodable \textit{from erasures}, an analog to the classical notion introduced by \cite{Guruswami2001ListDF}. We show that this particular code composition is able to correct from adversarial erasures even over qubits, while entirely removing the need for randomness in the encoding. 


\subsubsection{Keyless Quantum Authentication on Qubit-wise Channels}


Our second application of $\PMD$ codes is to designing quantum authentication codes \textit{without} a secret key.  

Quantum authentication codes were first introduced in \cite{barnum2002authentication}. Informally, they correspond to a protocol in which a sender (Alice) conveys a quantum message $\psi$ to a receiver (Bob) over some insecure quantum channel $\Lambda$, with the guarantee that Bob either receives a state close to $\psi$, or aborts $\bot$. 

\cite{barnum2002authentication} showed that, in general, sending an authenticated $k$ qubit message requires a secret key of at least $2k\cdot (1-o(1))$ bits shared between Alice and Bob. In fact, they show that any quantum authentication code must also be a quantum ``encryption scheme", meaning that an adversary $\Lambda$ who does not know the secret key, learns nothing about the message state. As otherwise, an all-powerful quantum adversary $\Lambda$ could extract partial information about the message, and thereby undetectably change the code-state. The motivating question we ask here is: 

\textit{Are there simpler adversarial channels $\Lambda$ for which quantum authentication is possible without a secret key?}

The model we study in this paper is that of ``qubit-wise" channels, where $\Lambda = \otimes_{i\in [n]}\Lambda_i$. Informally, this corresponds to Alice sending each qubit of her $n$ qubit code-state to $n$ distinct, non-communicating and un-entangled parties. These parties may strategize ahead of time and decide on a nefarious combination of distinct channels $\Lambda_i\neq \Lambda_j$, but they must act on the code-state independently of each other. 

It should be clear that this task remains impossible classically. Indeed, in the absence of shared randomness, the $n$ parties can always collude ahead of time, and substitute the entire message with a valid encoding of any other pre-agreed message $\hat{m}$. Bob will be none the wiser, and will decode to $\hat{m}$ without noticing that Alice's message has been completely replaced. Nonetheless, we show that in the quantum setting the scenario is drastically different:

\begin{theorem}\label{theorem:auth-results}
    For every sufficiently large $n\in \mathbb{N}$, there exists a Monte Carlo construction of an $n$ qubit quantum authentication code for qubit-wise channels, without a secret key, of rate $1-O(\log^{-1}n)$ and error $\epsilon \leq 2^{-\Tilde{\Omega}(n)}$. The construction succeeds with probability $1-2^{-\Tilde{\Omega}(n)}$.
\end{theorem}

The key tool in our code construction is a classical non-malleable code against bit-wise tampering functions \cite{Dziembowski2010}. Classical non-malleable codes are a relaxation of authentication and error correcting codes, where Bob is tasked with decoding Alice's message $m$ to either the original message $m$, rejection $\bot$, or a completely unrelated value $\Tilde{m}$. In contrast to authentication and error correction, non-malleable codes are much more versatile and can be constructed in a number of limited-adversarial settings, even without a secret key. 

%Our code construction is based on a combination of PMD codes,  stabilizer codes, and classical non-malleable codes for bit-wise tampering functions \cite{Dziembowski2010}. A classical non-malleable code is a relaxation of an authentication or error correcting code, where Bob is tasked with decoding Alice's message $m$ to either the original message $m$, rejection $\bot$, or a completely unrelated value $\Tilde{m}$. In contrast to authentication and error correction, non-malleable codes are much more versatile and can be constructed in a number of limited-adversarial settings, even without a secret key. 

Our code construction combines non-malleable codes with PMD codes and stabilizer codes, and is inspired by the design of a classical bit-wise non-malleable code by \cite{Cheraghchi2013NonmalleableCA}. In this application, our main technical contribution draws ideas from the quantum circuit lower bounds by \cite{Anshu2020CircuitLB}, to show how to use entanglement to evade the previously mentioned ``substitution" attack, and detect adversarial tampering without a secret key. 

Subsequent to the posting of this work, Boddu, Jain, Goyal and Ribeiro defined an interesting notion of a \textit{quantum} non-malleable code, and presented a construction in the split-state model with entangled adversaries. While our qubit-wise adversarial model is strictly weaker than theirs, we emphasize that our tamper detection guarantees are fundamentally stronger than any form of classical or quantum non-malleability.

%Our main result is inspired by a construction of bit-wise non-malleable codes by \cite{Cheraghchi2013NonmalleableCA}, and leverages quantum code concatenation with pseudorandomness to achieve the near-optimal rate. However, we emphasize that our result is fundamentally stronger than any form of classical or quantum non-malleability (for qubit-wise channels). One of our main technical contributions draws ideas from the quantum circuit lower bounds by \cite{Anshu2020CircuitLB}, to show how to evade the previously mentioned ``substitution" attack, and indeed achieve authentication without a secret key. 

%We note two interesting remarks about \Cref{theorem:auth-results}. First, it gives a simple example of a task in quantum communication which is provably impossible classically, and shows conclusive evidence that our motivating question is True. Second, it questions the role of encryption in quantum authentication against restricted adversaries. Not only does our construction have minimal redundancy (rate approaching $1$), but the amount of randomness Alice uses to generate her mixed-state code-states is \textit{sublinear} in the block-length $n$. 


\subsection{Related Work}
\label{section:related}

\textbf{Tamper-detection codes and Secret Sharing}

Our work is inspired by constructions of classical secret sharing schemes from ideas in tamper-resilient cryptography \cite{Cramer2001OnTC, Cramer2008DetectionOA, Cramer2015OptimalAM, Cramer2015LinearSS, Lin2018SecretSW}. A key ingredient in that line of work is the concept of an algebraic manipulation detection (AMD) code \cite{Cramer2008DetectionOA}. Simply put, an ``algebraic manipulation" is a form of adversarial data tampering, without prior knowledge of the data values. For instance, if our data is a value $x$ in a group $\mathcal{G}$, then an ``algebraic manipulation" corresponds to adding some value $\delta\in \mathcal{G}$ (without knowing $x$), resulting in $x+\delta$. An AMD code corresponds to an encoding of data into $\mathcal{G}$, in a way that any algebraic manipulation $\delta\neq 0$ is detected with high probability. 

%Most related to our work are the results of \cite{Cramer2015LinearSS}, who showed how to construct robust secret sharing schemes from the composition of AMDs and list-decodable codes. Although we focus on erasures, our abstract reduction from erasure decoding to list decoding and PMDs is a direct quantum analog of their work.

%Our work is inspired by constructions of classical secret sharing schemes from ideas in tamper-resilient cryptography \cite{Cramer2001OnTC, Cramer2008DetectionOA, Cramer2015OptimalAM, Cramer2015LinearSS, Lin2018SecretSW}. A key ingredient in that line of work is the concept of an algebraic manipulation detection (AMD) code, introduced by \cite{Cramer2008DetectionOA}. Simply put, an ``algebraic manipulation" is a form of adversarial data tampering, without prior knowledge of the data values. For instance, if our data is a value $x$ in some abelian group $\mathcal{G}$, then an ``algebraic manipulation" corresponds to adding some value $\delta\in \mathcal{G}$ (without knowing $x$), resulting in $x+\delta$. An AMD code corresponds to an encoding of source data into $\mathcal{G}$, in a way that any algebraic manipulation $\delta\neq 0$ is detected with high probability. 

%Most related to our work are the results of \cite{Cramer2015LinearSS}, who showed how to construct robust secret sharing schemes from the composition of AMDs and list-decodable codes. Although we focus on erasures, our abstract reduction from erasure decoding to list decoding and PMDs is a direct quantum analog of their work. Informally, they reason that the list-decodable code provides a short list of candidate codewords for the original secret, each one of which is a candidate AMD codeword. The decoder can then check each of these candidate AMD codewords, and with high probability, only one of which will be correct. 

\cite{Boddu2021TamperDA} were the first to explore tamper-detection codes in the quantum setting. Their work focused on the concept of a ``Unitary Tamper Detection Code", a quantum code which can faithfully detect any tampering from a family of unitary operators. Among other results, they constructed explicit quantum codes for classical messages which could detect arbitrary Pauli errors, which they referred to as ``Quantum AMDs". Our PMDs arose as a natural generalization to quantum messages, albeit our techniques depart significantly. 

\textbf{Non-Malleable Codes}

%The key tool we use to design our authentication codes are classical non-malleable codes \cite{Dziembowski2010}, a relaxation of authentication codes and error correcting codes. In a non-malleable code, Bob is tasked with decoding Alice's message $m$ to either the original message $m$, rejection $\bot$, or a completely unrelated value $\Tilde{m}$. In contrast to authentication and error correction, non-malleable codes are much more versatile and can be constructed in a number of limited-adversarial settings, even without a secret key. 

The first construction of an efficient non-malleable code by \cite{Dziembowski2010} was for ``bit-wise" tampering functions, which is the conceptual classical analog to the qubit-wise channels we study. A series of works then built on their results by developing explicit and ``minimal redundancy" (rate $1-o(1)$) constructions \cite{Cheraghchi2013NonmalleableCA, nm-permutations, nm-rate-optimizing}. Qualitatively, our construction of authentication codes is inspired by \cite{Cheraghchi2013NonmalleableCA}, who combined a ``concatenated" non-malleable code with a pseudorandom permutation. The secret key for the permutation was then itself hidden back into the code, using a smaller, sub-optimal non-malleable code. Outside of the bit-wise setting, other notable examples of non-malleable codes include the well studied ``split-state'' model \cite{DKO13,adl14, KOS17, ASK22, split-state-review}, as well as AC$^0$ \cite{marshalllowdepth} and poly-sized \cite{marshalllarge} circuits. 

%Subsequent to our work, Boddu, Jain, Goyal and Ribeiro defined a notion of a quantum non-malleable code. Informally, in their definition the receiver Bob is tasked with either outputting the original quantum message $\psi$, or a fixed  message $\sigma$ (decoupled from any side-entanglement). 


\textbf{Approximate Quantum Error Correction}

\cite{Leung1997ApproximateQE} were the first to showcase the benefits of approximate error correction to quantum communication. They constructed a 4 qubit code which could correct a single amplitude dampening error, violating the ``Hamming bound" for quantum codes based on the Pauli basis. Several results then studied conditions in which approximate quantum error correction is even possible \cite{Barnum2000ReversingQD, SW02, Devetak2005ThePC, Kretschmann2006TheIT, Bny2009ConditionsFT, MN10, MN12, BO10, Hayden2017ApproximateQE}.

In this context, most related to our work are the results of \cite{Crpeau2005ApproximateQE, Leung2006CommunicatingOA, Bergamaschi2022ApproachingTQ}, who studied the adversarial error channel. While it is well known consequence of the Knill-Laflamme conditions \cite{Knill1996TheoryOQ} that no exact quantum code can correct from more than $n/4$ adversarial errors, \cite{Crpeau2005ApproximateQE} constructed approximate quantum codes which could correct $(n-1)/2$ adversarial errors, all the way up to the no-cloning bound! Their codes relied on an insightful combination of quantum error correction, quantum authentication, and classical secret sharing, but came at a cost of an exponentially large alphabet size and assymptotically decaying rate. 

\cite{Leung2006CommunicatingOA, Bergamaschi2022ApproachingTQ} address these issues using the list-decoding of stabilizer codes. \cite{Leung2006CommunicatingOA} presented a quantum code over qubits which beat the quantum GV bound, albeit relied on an inefficient decoding algorithm, and a secret key shared between sender and receiver. \cite{Bergamaschi2022ApproachingTQ} showed how to efficiently approach the quantum Singleton bound over (large, but) constant-sized alphabets, by combining purity testing codes and classical secret sharing with efficient constructions of list-decodable stabilizer codes. 

While in this work we share many of the same tools as \cite{Bergamaschi2022ApproachingTQ}, what fundamentally distinguishes our approaches to approximate quantum error correction is that (1) our goal is to design codes over qubits, and (2) we attempt to correct from a number of (erasure) errors much larger than the underlying code distance. Thereby, we cannot rely on techniques such as ``code-blocking" to hide shared randomness back into the code\footnote{As similarly done by \cite{Crpeau2005ApproximateQE} and \cite{Hayden2017ApproximateQE} to approach the no-cloning bound.}, nor can we leverage ``privacy" by relying on the exact local-indistinguishability of the code. 

\textbf{Quantum Secret Sharing}

\cite{Gottesman1999TheoryOQ, Cleve1999HOWTS, Smith2000QuantumSS, Crpeau2005ApproximateQE} showed that exact and approximate quantum error correction and quantum secret sharing are deeply connected. In a quantum $(n, t)$-threshold secret sharing scheme, a secret quantum state is encoded into $n$ shares such that any $t$ can be used to reconstruct the secret, but any $\leq t-1$ contain no information about the secret. By definition, this is already a quantum error correcting code, and \cite{Cleve1999HOWTS} noted that the converse is also true. Via the information-disturbance paradigm, even approximately correcting from quantum erasures implies the approximate privacy of the erased subset \cite{Kretschmann2006TheIT}.

A natural extension to threshold secret sharing is the concept of a $(n, t, p)$ \textit{ramp} secret sharing scheme, where the ``reconstruction" and ``privacy" thresholds are distinct. Any $t$ suffice to reconstruct the secret, but no $p$ of them reveal any information. Our result in \cref{theorem:main} can be understood as a near-optimal quantum ramp secret sharing scheme encoding secrets of $r\cdot n$ qubits into $n$ binary shares, where $t = (\frac{1+r}{2}+\gamma)\cdot n, p= (\frac{1-r}{2}-\gamma)\cdot n$, with recovery and privacy error $2^{-\Omega(\gamma\cdot n)}$.









==> 9-designs.tex <==


\section{PMD codes from $t$-designs}

\subsection{Background on $t$-designs}

\subsubsection{Definitions}

Informally, a $t$ design is a distribution over unitary matrices whose first $t$ moments emulate those of the Haar measure. 

\begin{definition}
    Let $\nu$ be a distribution on the unitary group $U(d)$. $\nu$ is a unitary $t$ design if 
    \begin{equation}
        \mathbb{E}_\nu\bigg[U^{\otimes t}\rho (U^\dagger)^{\otimes t}\bigg] = \mathbb{E}_\mathbb{H}\bigg[U^{\otimes t}\rho (U^\dagger)^{\otimes t}\bigg]
    \end{equation}

    \noindent For all $d^t\times d^t$ complex matrices $\rho$.
\end{definition}

To instantiate our constructions, we require a notion of an approximate unitary designs. To do so, we express the notion of approximation in terms polynomials over the matrix elements of the unitaries $U$.

\begin{definition}
    A monomial $M(U)$ in the matrix entries of $U$ is said to be a ``balanced" degree $k$ monomial if it contains $k$ conjugated elements and $k$ un-conjugated elements. 
\end{definition}

\begin{definition}
    $\mu$ is an $\epsilon$ approximate unitary $t$ design if for all balanced monomials $M$ of degree $\leq t$, 

    \begin{equation}
        |\mathbb{E}_\nu M(U) - \mathbb{E}_\mathbb{H} M(U)|\leq \epsilon\cdot d^{-t}
    \end{equation}
\end{definition}

Before moving on, we briefly recall a simple property of expectations over 2 designs. 

\begin{definition}
    The swap operator $F$ on a bipartite Hilbert space $\mathcal{H}_A\otimes \mathcal{H}_B$ both of dimension $q$ is defined by
    \begin{equation}
        F = \sum_{x, y\in [q]} \ket{x}\bra{y}_A\otimes \ket{y}\bra{x}_B
    \end{equation}
\end{definition}

\begin{fact} \label{fact:haarfact}
    If $V$ is a $q$-dimensional unitary drawn from the Haar measure over $U(q)$ and $\rho$ is a $q^2\times q^2$ Hermitian operator, then
    \begin{equation}
        \mathbb{E}_{V\leftarrow \mathbb{H}}[V^{\otimes 2} \rho V^{\dagger, \otimes 2}] = \frac{\text{Tr}[\rho]-q^{-1}\text{Tr}[\rho F]}{q^2-1} \cdot \mathbb{I} + \frac{\text{Tr}[\rho F] - q^{-1}\text{Tr}[\rho]}{q^2-1} \cdot F
    \end{equation}
    where $F$ is the Swap operator. 
\end{fact}

\subsubsection{Constructions}


\subsubsection{Large Deviation bounds for the Haar Measure}

\begin{definition}
    The Lipschitz constant with respect to the Euclidean norm for a function $f$ is the minimum $\eta$ such that
    \begin{equation}
        |f(U)-f(V)|\leq \eta\cdot \|U-V\|_2
    \end{equation}
\end{definition}

\begin{fact}
    [Levy's Lemma, \cite{Ledoux2001TheCO}]\label{fact:levy} Let $f$ be an $\eta$-Lipschitz function on $U(d)$ with mean $\mathbb{E} f$. Then, 

    \begin{equation}
        \mathbb{P}_{V\leftarrow \mathbb{H}}\big[|f(V)-\mathbb{E}f|\geq \delta\big] \leq 4\cdot \exp\big[- \frac{C_1d\delta^2}{\eta^2}\big]
    \end{equation}

    \noindent Where $C_1$ can be taken to be $\frac{2}{9\pi^3}$.
\end{fact}

We can now state the large deviation bounds for $t$ designs by \cite{Low2009LargeDB}. Typically, Levy's lemma is used to find some concentration bound for polynomial functions of Haar random unitaries $U$, which can then be turned into a moment bound for $t$-designs as below.

\begin{theorem}[\cite{Low2009LargeDB}]\label{theorem:low}
    Let $f$ be a polynomial of degree $K$ over $U(d)$, written as $f(V) = \sum \alpha_i M_i(V)$ where $M_i$ are monomials in the matrix entries of $V$, and let $\alpha(f) = \sum_i |\alpha_i|$ be its sum of coefficients. Suppose that $f(V)$ has mean $\mu = \mathbb{E}f$ and concentrates around the mean for Haar random $V$: 
    \begin{equation}
        \mathbb{P}_{V\leftarrow \mathbb{H}}\big[|f(V)-\mathbb{E}f|\geq \delta\big] \leq 2^{-a\cdot  \delta^2}
    \end{equation}
    
    \noindent For some $a$. Then, if $\nu$ is an $\epsilon$-approximate $t$-design, for every integer $m\leq t/2K$ we have
    \begin{equation}
        \mathbb{P}_{V\leftarrow \nu}\big[|f(V)-\mathbb{E}f|\geq \delta\big]\leq \bigg(\frac{m}{a\cdot \delta^2}\bigg)^m + \frac{\epsilon}{d^t}\cdot \bigg(\frac{\alpha(f) + \mu}{\delta}\bigg)^{2m}
    \end{equation}
\end{theorem}
